Cocon: Computation in Contextual Type Theory

We describe a Martin-L\"of style dependent type theory, called Cocon, that allows us to mix the intensional function space that is used to represent higher-order abstract syntax (HOAS) trees with the extensional function space that describes (recursive) computations. We mediate between HOAS representations and computations using contextual modal types. Our type theory also supports an infinite hierarchy of universes and hence supports type-level computation -- thereby providing metaprogramming and (small-scale) reflection. Our main contribution is the development of a Kripke-style model for Cocon that allows us to prove normalization. From the normalization proof, we derive subject reduction and consistency. Our work lays the foundation to incorporate the methodology of logical frameworks into systems such as Agda and bridges the longstanding gap between these two worlds.

==> completness.tex <==
\begin{theorem}[Completeness]\label{lem:SemComplete}
If $\Gamma \Vdash t = t' : \tau$ then $\Gamma \vdash t : \tau$ and
$\Gamma \vdash t' : \tau$ and
$\Gamma \vdash t \equiv t' : \tau$ and
$\Gamma \vdash \tau$.
\end{theorem}


%%%Need to prove that Gamma |- t : tau => Gamma |-tau
%%%Need to prove that Gamma |-w = w' : y:tau1 -> tau2

\begin{proof}
  \pcase{$\Gamma \Vdash t = t' : [T]$ }\\
  \prf{$\Gamma \vdash t \whnf w   : [T]$ \hfill by assumption}
  \prf{$\Gamma \vdash t : [T]$ \hfill by definition of $\Gamma \vdash t \whnf w   : [T]$ }
  \prf{$\Gamma \vdash t \equiv w : [T]$\hfill by definition of $\Gamma \vdash t \whnf w   : [T]$ }
  \prf{$\Gamma \vdash t' \whnf w'   : [T]$ \hfill by assumption}
  \prf{$\Gamma \vdash t' : [T]$ \hfill by definition of $\Gamma \vdash t' \whnf w'   : [T]$ }
  \prf{$\Gamma \vdash t' \equiv w' : [T]$\hfill by definition of $\Gamma \vdash t' \whnf w'   : [T]$ }
  \prf{$\Gamma\vdash t \equiv t' : [T]$ \hfill since  $\Gamma \vdash w \equiv w' : [T]$ and by transitivity and symetry of the equivalence}\\
    %%%MISS Gamma |-[T]
  \pcase{$\Gamma \Vdash t = t' : (y:\tau_1) \arrow \tau_2$ }\\
  \prf{$\Gamma \vdash t \whnf w   : (y:\tau_1) \arrow \tau_2$ \hfill by assumption}
  \prf{$\Gamma \vdash t : (y:\tau_1) \arrow \tau_2$ \hfill by definition of $\Gamma \vdash t \whnf w   : (y:\tau_1) \arrow \tau_2$ }
  \prf{$\Gamma \vdash t \equiv w : (y:\tau_1) \arrow \tau_2$\hfill by definition of $\Gamma \vdash t \whnf w   : (y:\tau_1) \arrow \tau_2$ }
  \prf{$\Gamma \vdash t' \whnf w'   : (y:\tau_1) \arrow \tau_2$ \hfill by assumption}
  \prf{$\Gamma \vdash t' : (y:\tau_1) \arrow \tau_2$ \hfill by definition of $\Gamma \vdash t' \whnf w'   : (y:\tau_1) \arrow \tau_2$ }
  \prf{$\Gamma \vdash t' \equiv w' : (y:\tau_1) \arrow \tau_2$\hfill by definition of $\Gamma \vdash t' \whnf w'   : (y:\tau_1) \arrow \tau_2$ }
\end{proof}



\subsection{proof}




\begin{lemma}
  If $\Gamma \vdash t  :\tau$ then $\Gamma \vdash \tau$ \\
  If $\Gamma \vdash C : T$ then $\Gamma \vdash T$.\\
  If $\Gamma \vdash M : A$ then $\Gamma \vdash A: \lftype$
\end{lemma}

\begin{proof}
  I will only explain the proof when there are difficulties to prove it just with the induction.\\
  By induction on the structure of the derivation :\\
  \pcase{\ibnc{y:\tau \in \Gamma}{\vdash\Gamma}{\Gamma \vdash y : \tau}{}}\\
  \prf{$\Gamma = \Gamma_1 , y: \tau,\Gamma_2$ \hfill since $y : \tau \in \Gamma $}\\
  \prf{$\Gamma_1 \vdash \tau$ \hfill since $\vdash \Gamma$}\\
  \prf{$\Gamma \vdash_w \rho :\Gamma_1$ \hfill by lemma \ref{?}}\\
  \prf{$\Gamma \vdash \{\rho\}\tau$ \hfill by weakening theorem}\\
  \prf{$\Gamma \vdash \tau$ \hfill since $\tau = \{\rho\}\tau$}\\
  %
  \pcase{\ibnc{\Gamma \vdash t : (y:\tau_1) \arrow \tau_2}{\Gamma \vdash s : \tau_1}{\Gamma \vdash t~s : \{s/y\}\tau_2}{}}\\
  \prf{$\Gamma \vdash  (y:\tau_1) \arrow\tau_2$ \hfill by IH}\\
  \prf{$\Gamma, y:\tau_1 \vdash \tau_2$ \hfill by inversion}\\
  \prf{$\Gamma \vdash \{s/y\}\tau_2$ \hfill with the second premisse and by lemma \ref{}}
  %
  \pcase{\ibnc{\Gamma \vdash t : \tau'}{\Gamma \vdash \tau' \equiv \tau}{\Gamma \vdash t : \tau}{}}
  \prf{TO DO}
%TODO : gamma|- tau = tau' -> gamma|- tau
  %
  \pcase{\icnc{\Gamma \vdash \trec{\R}{\tm}{\psi,y.\tau} : (\psi : \cbox{\tmctx}) \arrow (y:\cbox{\psi \vdash \tm}) \arrow \tau}{\Gamma \vdash \Psi : \tmctx}{\Gamma \vdash t : \cbox{\Psi \vdash \tm}}{\Gamma \vdash \trec{\R}{\tm}{\psi,y.\tau}~\cbox{\Psi}~t :  \{\cbox \Psi/\psi, t/y\}\tau}{}}
    \prf{$\Gamma \vdash (\psi : \cbox{\tmctx}) \arrow (y:\cbox{\psi \vdash \tm}) \arrow \tau$\hfill by IH}
    \prf{$\Gamma,\psi : \cbox{\tmctx}, y:\cbox{\psi \vdash \tm} \vdash \tau $ \hfill by inversion}
    \prf{$\Gamma \vdash \cbox \Psi : \cbox \tmctx$ \hfill by rule and premise}
    \prf{$\Gamma, y : \cbox{\Psi\vdash \tm} \vdash \{\Psi / \psi\}\tau$ \hfill by Lemma \ref{}} \prf{$\Gamma \vdash \{\Psi/\psi, t/y\}\tau$ \hfill by Lemma \ref{}}
    %
    \pcase{$\Gamma \vdash \tmrec {\psi,y.\tau} {\psi,p \mto t_v} {\psi, m, n, f_n, f_m \mto t_{\mathsf{app}}} {\psi, m, f_m \mto t_{\clam}} : (\psi : \cbox{\tmctx}) \arrow (y:\cbox{\psi \vdash \tm}) \arrow \tau$}
    \prf{TO DO}
    \prf{$\Gamma, \psi : \cbox{\tmctx}, y:\cbox{\psi \vdash \tm} \vdash \tau$ \hfill ???????}
    \prf{$\Gamma, \psi : \cbox{\tmctx} \vdash (y:\cbox{\psi \vdash \tm}) \arrow \tau$ \hfill by rule}
    \prf{$\Gamma \vdash (\psi : \cbox{\tmctx}) \arrow (y:\cbox{\psi \vdash \tm}) \arrow \tau$ \hfill by rule}
% \Gamma & \vdash & t : \cbox{\Psi \vdash \tm}\\[0.5em]
%\Gamma, \phi:\cbox{\tmctx}, m:\cbox{~\unboxc{\phi}, x:\tm \vdash \tm}, f_m:\{\cbox{~\unboxc{\phi}, x:\tm}/\psi, m /y \} \tau & \vdash & t_{\clam} : \{\phi/\psi, \cbox{~\unboxc{\phi} \vdash \clam~\lambda x.\unbox{m}{(\id_{\unboxc{\phi}}, x)}~} / y\}\tau\\[0.5em]
%\Gamma, \psi:\cbox{\tmctx}, m:\cbox{~\unboxc{\psi} \vdash \tm}, n:\cbox{~\unboxc{\psi} \vdash \tm}, f_m: \{m/y\}\tau, f_n: \{n/y\}\tau & \vdash & t_{\mathsf{app}} : \{\cbox{~\unboxc{\psi} \vdash\capp~\unbox{m}{\id_{\unboxc{\psi}}}~\unbox{n}{\id_{\unboxc{\psi}}}}/y\}\tau
%\Gamma, \psi:\cbox{\tmctx}, p:\cbox{~\unboxc{\psi} \vdash_\# \tm} & \vdash & t_v : \{p / y\}\tau
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \pcase{\ianc{\Gamma ; \Psi \vdash M : A}{\Gamma \vdash (\Psi \vdash M) : (\Psi \vdash A)}{}}
  \prf{$\Gamma ; \Psi \vdash A : \lftype$ \hfill by IH}
  \prf{ $\Gamma \vdash \Psi \ctx$ \hfill by Lemma \ref{lm :fulllfctxwf} }
  \prf{ $\Gamma \vdash (\Psi\vdash A)$ \hfill by rule}
  %
  \pcase{\ianc{\Gamma \vdash t : \cbox \tmctx }{\Gamma \vdash \unboxc{t} : \tmctx}{}}
  \prf{$\Gamma \vdash \tmctx$ \hfill by IH}
  \prf{$\Gamma \vdash \cbox \tmctx$ \hfill by rule}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \pcase{\ianc{\Gamma ; \Psi, x{:}A \vdash M : B}{\Gamma ; \Psi \vdash \lambda x.M : \Pityp x A B}{}}
  \prf{$\Gamma ; \Psi, x{:}A \vdash B : \lftype$ \hfill by IH}
  \prf{$\Gamma \vdash \Psi, x : A \ctx$ \hfill by Lemma \ref{lm :fulllfctxwf}}
  \prf{$\Gamma ; \Psi \vdash A : \lftype $ \hfill by inversion}
  \prf{$\Gamma ; \Psi \vdash \Pityp x A B : \lftype$ \hfill by rule}
  %
  \pcase{\ibnc{\Gamma \vdash t : [\Phi \vdash A] ~\mbox{or}~\Gamma \vdash t : [\Phi \vdash_\# A]}{\Gamma; \Psi \vdash \sigma : \Phi}{\Gamma ; \Psi \vdash \unbox t {\sigma} : [\sigma]A}{}}
  \prf{$\Gamma \vdash [\Phi \vdash A] ~\mbox{or}~\Gamma \vdash [\Phi \vdash_\# A]$ \hfill by IH }
  \prf{$\Gamma \vdash \Phi \vdash A ~\mbox{or}~\Gamma \vdash \Phi \vdash_\# A $ \hfill by inversion }
  \prf{$\Gamma; \Phi \vdash  A : \lftype ~\mbox{or}~\Gamma  \Phi \vdash_\# A : \lftype $ \hfill by inversion }
  \prf{$\Gamma; \Psi \vdash \sigma : \Phi$ \hfill by assumption}
  \prf{$\Gamma ; \Psi \vdash [\sigma]A$ \hfill by Lemma \ref{} and $\vdash_\#$ is a restriction of $\vdash$}
  %
  \pcase{\ibnc{\Gamma\vdash \Psi : \ctx}{x:A \in \Psi}{\Gamma ; \Psi \vdash x : A}{}}
  \prf{$\Gamma\vdash \Psi', x:A :\ctx$ \hfill with $\Psi = \Psi', x :A, \Psi''$ by inversion}
  \prf{$\Gamma ; \Psi' \vdash A :\lftype$ \hfill by inversion}
  \prf{$\Gamma; \Psi \vdash A : \lftype $ \hfill by Lemma \ref{lm:extlfctx}(multiple times)}
  %
  \pcase{\ibnc{\Gamma ; \Psi \vdash M : \Pityp x A B}{\Gamma ; \Psi \vdash N : A}{\Gamma ; \Psi \vdash M~N : [N/x]B}{}}
  \prf{$\Gamma ; \Psi \vdash \Pityp x A B : \lftype$ \hfill by IH}
  \prf{$\Gamma ; \Psi, x: A \vdash B$ \hfill by inversion}
  \prf{$\Gamma ; \Psi \vdash [N/x]B$ \hfill by lemma \ref{}}
  %
  \pcase{\ibnc{\Gamma\vdash \Psi : \ctx}{\mathsf{lam}{:} \Pityp y {(\Pityp x \tm \tm)} \tm \in \Sigma}{\Gamma ; \Psi \vdash \mathsf{lam}{:} \Pityp y {(\Pityp x \tm \tm)} \tm}{}}
  \prf{$\Gamma;\Psi \vdash \tm : \lftype$ \hfill by rule}
  \prf{$\Gamma \vdash \Psi, x{:}\tm : \ctx$ \hfill by rule}
  \prf{$\Gamma; \Psi, x {:}\tm \vdash  \tm : \lftype$ \hfill by Lemma \ref{lm:extlfctx}}
  \prf{$\Gamma;\Psi\vdash \Pityp x \tm \tm : \lftype$ \hfill by rule}
  \prf{$\Gamma \vdash \Psi, y : \Pityp x \tm \tm : \ctx$ \hfill by rule}
  \prf{$\Gamma; \Psi,y: \Pityp x \tm \tm \vdash \tm : \lftype$ \hfill by Lemma \ref{}}
  \prf{$\Gamma; \Psi \vdash \Pityp y (\Pityp x \tm \tm ) \tm : \lftype$ \hfill by rule}
  %
  \pcase{\ibnc{\Gamma\vdash \Psi : \ctx}{\mathsf{app}{:} \Pityp x \tm {\Pityp y \tm \tm} \in \Sigma}{\Gamma ; \Psi \vdash \mathsf{app}{:} \Pityp x \tm {\Pityp y \tm \tm}}{}}
 \prf{$\Gamma;\Psi \vdash \tm : \lftype$ \hfill by rule}
  \prf{$\Gamma \vdash \Psi, y{:}\tm : \ctx$ \hfill by rule}
  \prf{$\Gamma; \Psi, y {:}\tm \vdash  \tm : \lftype$ \hfill by Lemma \ref{lm:extlfctx}}
  \prf{$\Gamma;\Psi\vdash \Pityp y \tm \tm : \lftype$ \hfill by rule}
  \prf{$\Gamma \vdash \Psi, x : \tm : \ctx$ \hfill by rule}
  \prf{$\Gamma; \Psi,x:\tm \vdash \Pityp y \tm \tm : \lftype$ \hfill by Lemma \ref{}}
  \prf{$\Gamma; \Psi \vdash \Pityp x \tm (\Pityp y \tm \tm ): \lftype$ \hfill by rule}
  %
  \pcase{\ibnc{\Gamma ; \Psi \vdash M : B }{\Gamma ; \Psi \vdash A \equiv B : \lftype}{\Gamma ; \Psi \vdash M : A}{}}
  \prf{TODO}
\end{proof}









\begin{lemma}
  \begin{itemize}
  \item If $\Gamma \vdash \tau' \equiv \tau$ then $\Gamma \vdash \tau$ and $\Gamma\vdash \tau'$
  \item If $\Gamma ; \Psi \vdash A \equiv B : \lftype$ then $\Gamma\vdash A :\lftype$ and $\Gamma \vdash B : \lftype$
  \item If $\Gamma \vdash C\equiv C': T$ then $\Gamma \vdash C :T$ and $\Gamma\vdash C' : T$
  \end{itemize}
\end{lemma}

\begin{proof}
  \pcase{\ibnc{\Gamma \vdash t_1 \equiv s_1 : (y:\tau_1) \arrow \tau_2}{\Gamma \vdash t_2 \equiv s_2 : \tau_1}{\Gamma \vdash t_1~t_2 \equiv s_1~s_2 : \{t_2/y\}\tau_2}{}}
  \prf{TODO}
  %
  \pcase{\icnc{\Gamma \vdash \trec{\R}{\tm}{\psi,y.\tau} \equiv \trec{\R'}{\tm}{\psi,y.\tau} : (\psi : \cbox{\tmctx}) \arrow (y:\cbox{\psi \vdash \tm}) \arrow \tau}{\Gamma \vdash \Psi \equiv \Phi : \tmctx}{\Gamma \vdash t \equiv s : \cbox{\Psi \vdash \tm}}{\Gamma \vdash \trec{\R}{\tm}{\psi,y.\tau}~\cbox{\Psi}~t \equiv \trec{\R'}{\tm}{\psi,y.\tau}~\cbox{\Phi}~s :  \{\cbox \Psi/\psi, t/y\}\tau}{} }


  \prf{$\Gamma \vdash \trec{\R}{\tm}{\psi,y.\tau} : (\psi : \cbox{\tmctx}) \arrow (y:\cbox{\psi \vdash \tm}) \arrow \tau$ \hfill by IH}
  \prf{$\Gamma \vdash \trec{\R'}{\tm}{\psi,y.\tau} : (\psi : \cbox{\tmctx}) \arrow (y:\cbox{\psi \vdash \tm}) \arrow \tau$ \hfill by IH}
  \prf{$\Gamma \vdash \Psi : \tmctx$ \hfill by IH}
  \prf{$\Gamma \vdash \Phi : \tmctx$ \hfill by IH}
  \prf{$\Gamma \vdash t \equiv s : \cbox{\Psi \vdash \tm}$ \hfill by IH}
  \prf{$\Gamma \vdash s : \cbox{\Psi \vdash \tm}$ \hfill by IH}
  \prf{$\Gamma;\Psi\vdash \tm :\lftype$ \hfill by rule}
  \prf{$\Gamma;\Psi\vdash \tm \equiv \tm :\lftype$ \hfill by rule}
  \prf{$\Gamma \vdash (\Psi \vdash \tm) \equiv (\Phi\vdash \tm)$\hfill by rule}
  \prf{$\Gamma \vdash \cbox{\Psi \vdash \tm} \equiv \cbox{\Phi\vdash \tm}$\hfill by rule}
  \prf{$\Gamma \vdash s : \cbox{\Phi \vdash \tm}$ \hfill by rule}
  \prf{$\Gamma \vdash \trec{\R}{\tm}{\psi,y.\tau}~\cbox{\Psi}~t  :  \{\cbox \Psi/\psi, t/y\}\tau$ \hfill by rules}
  \prf{$\Gamma \vdash \trec{\R'}{\tm}{\psi,y.\tau}~\cbox{\Phi}~s :  \{\cbox \Phi/\psi, s/y\}\tau$ \hfill by rules}





  \prf{$\Gamma \vdash \trec{\R'}{\tm}{\psi,y.\tau}~\cbox{\Phi}~s :  \{\cbox \Psi/\psi, t/y\}\tau$ \hfill ??????}








  %
  \infer{\Gamma \vdash \tmrec{\psi,y .\tau} {\psi,p \mto t_v} {\psi,m,n,f_m,f_n \mto t_{\mathsf{app}}} {\psi, m, f_m \mto t_{\clam}} t
    \equiv \tmrec{\psi,y.\tau'} {\psi,p \mto s_v} {\psi, m, n, f_m, f_n \mto s_{\mathsf{app}}} {\psi, m, f_m \mto s_{\clam}} s :(\psi : \cbox{\tmctx}) \arrow (y:\cbox{\psi \vdash \tm}) \arrow \tau }
        {
          \begin{array}{l@{~}l@{~}l}
            \Gamma \vdash \Psi : \tmctx \\[0.5em]
            % \Gamma; \Psi \vdash M : \tm \\[0.5em]
            \Gamma, \psi:\cbox{\tmctx}, y :\cbox{\unboxc{\phi} \vdash \tm} & \vdash & \tau \equiv \tau'  : \kind \\[0.5em]
            \Gamma & \vdash & t \equiv s : \cbox{\Psi \vdash \tm} \\[0.5em]
            \Gamma,
            \phi:\cbox{\tmctx},
            m:\cbox{~\unboxc{\phi}, x:\tm \vdash \tm},
            f_m:\{\cbox{~\unboxc{\phi}, x:\tm}/\psi, m /y \} \tau & \vdash & t_{\clam} \equiv s_{\clam} :
            \{\phi/\psi, \cbox{~\unboxc{\phi} \vdash \clam~\lambda x.\unbox{m}{(\id_{\unboxc{\phi}}, x)}~} / y\}\tau\\[0.5em]
            \Gamma, \psi:\cbox{\tmctx}, m:\cbox{~\unboxc{\psi} \vdash \tm}, n:\cbox{~\unboxc{\psi} \vdash \tm}, f_m: \{m/y\}\tau, f_n: \{n/y\}\tau  & \vdash & t_{\mathsf{app}} \equiv s_{\mathsf{app}} : \{\cbox{~\unboxc{\psi} \vdash\capp~\unbox{m}{\id_{\unboxc{\psi}}}~\unbox{n}{\id_{\unboxc{\psi}}}}/y\}\tau
            \\[0.5em]
            \Gamma, \psi:\cbox{\tmctx}, p:\cbox{~\unboxc{\psi} \vdash_\# \tm} & \vdash & t_v \equiv s_v : \{p / y\}\tau
          \end{array}
        }
        %
        \pcase{\ibnc{\Gamma \vdash (\Psi \vdash P) \equiv (\Phi \vdash P') : (\Psi \vdash A)}{\Gamma ; \Psi \vdash P \equiv P' : A}{\Gamma \vdash \Psi \equiv \Phi : \ctx}{}}
        \prf{$\Gamma ; \Psi \vdash P : A$ \hfill by IH}
        \prf{$\Gamma ; \Psi \vdash P' : A$ \hfill by IH}
        % \prf{$\Gamma \vdash \Psi : \ctx$ \hfill by IH}
        %\prf{$\Gamma \vdash \Phi : \ctx$ \hfill by IH}
 \prf{$\Gamma \vdash (\Psi\vdash R) : (\Psi \vdash A)$ \hfill by rule}
 \prf{TO DO}





%
\pcase{\ibnc{\Gamma \vdash \Psi \equiv \Phi: \tmctx}{\Gamma; \Psi \vdash A \equiv \tm : \lftype}{\Gamma; \Psi \vdash A \equiv B : \lftype}{\Gamma \vdash \Psi, x:A \equiv \Phi, x:B : \tmctx}{}}
\prf{$\Gamma; \Psi \vdash B \equiv \tm : \lftype$ \hfill by symetry and transitivity of equivalence}
\prf{$\Gamma \vdash \Psi : \tmctx$ \hfill by IH}
\prf{$\Gamma \vdash \Phi : \tmctx$ \hfill by IH}
\prf{$\Gamma; \Psi \vdash A : \lftype$ \hfill by IH}
\prf{$\Gamma; \Psi \vdash B : \lftype$ \hfill by IH}
\prf{$\Gamma \vdash \Psi, x:A : \tmctx$\hfill by rule}
\prf{$\Gamma \vdash \Phi, x:B : \tmctx$\hfill by rule}






\end{proof}































\begin{lemma}
  \begin{itemize}
  \item If $\Gamma \vdash t \equiv t': \tau$ then $\Gamma \vdash t : \tau$ and $\Gamma \vdash t' : \tau$
  \item If $\Gamma \vdash \tau \equiv \tau'$ then $\Gamma \vdash \tau $ and $\Gamma \vdash \tau'$
  \item If $\Gamma \vdash C \equiv C' :T$ then $\Gamma \vdash C : T$ and $\Gamma \vdash C' :T$
  \item If $\Gamma \vdash T \equiv T'$ then $\Gamma \vdash T$ and $\Gamma \vdash T'$
  \item If $\Gamma \vdash \Psi \equiv \Psi' : \tmctx$ then $\Gamma \vdash \Psi : \tmctx$ and $\Gamma \vdash \Psi' : \tmctx$
  \item If $\Gamma \vdash \Psi \equiv \Psi' : \ctx$ then $\Gamma \vdash \Psi : \ctx$ and $\Gamma \vdash \Psi' : \ctx$
  \item If $\Gamma; \Psi \vdash \sigma \equiv \sigma' : \Phi$ then $\Gamma ; \Psi \vdash \sigma : \Phi$ and $\Gamma ; \Psi \vdash \sigma' : \Phi$
  \item If $\Gamma; \Psi \vdash M \equiv N : A$ then $\Gamma; \Psi \vdash M : A$ and $\Gamma; \Psi \vdash N : A$
  \item If $\Gamma ; \Psi \vdash A \equiv B : K$ then $\Gamma ; \Psi \vdash A : K$ and $\Gamma ; \Psi \vdash B : K$
  \item $\Gamma ; \Psi \vdash K \equiv K' : \lfkind $ then $\Gamma ; \Psi \vdash K : \lfkind $ and $\Gamma ; \Psi \vdash K' : \lfkind $
  \end{itemize}
\end{lemma}

\begin{proof}
  We use mutual induction.\\
  \pcase{\ibnc{\Gamma ; \Psi \vdash M_1 \equiv M_2 : \Pityp x A B}{\Gamma ; \Psi \vdash N_1 \equiv N_2 : A}{\Gamma ; \Psi \vdash M_1~N_1 \equiv M_2~N_2 : [N_1/x]B}{}}
  \prf{$\Gamma ; \Psi \vdash M_1 : \Pityp x A $ \hfill by IH on the first premisse}
  \prf{$\Gamma ; \Psi \vdash M_2 : \Pityp x A $ \hfill by IH on the first premisse}
  \prf{$\Gamma ; \Psi \vdash N_1 : A$ \hfill by IH on the second premisse}
  \prf{$\Gamma ; \Psi \vdash N_2 : A$ \hfill by IH on the second premisse}
  \prf{$\Gamma ; \Psi \vdash M_1~N_1 : [N_1/x]B$ \hfill by rules}
  \prf{$\Gamma ; \Psi \vdash M_2~N_2 : [N_2/x]B$ \hfill by rules}





\end{proof}












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\begin{proof}
  We use induction on the .....
  \pcase{\ianc{\Gamma ; \Psi \vdash M : \Pityp x A B}{\Gamma ; \Psi \vdash M \equiv \lambda x.M~x : \Pityp x A B}{}}
  \prf{$\Gamma ; \Psi \vdash M : \Pityp x A B$ \hfill by assumption}
  \prf{$\Gamma;\Psi \vdash \Pityp x A B : \lftype$\hfill by IH (part I)??????}
  \prf{$\Gamma; \Psi, x:A \vdash B$ \hfill by inversion} %sure ??
  \prf{$\Gamma\vdash \Psi,x:A : \ctx$ \hfill by lemma \ref{lm :fulllfctxwf}}
  \prf{$\Gamma ; \Psi,x :A \vdash M : \Pityp x A B$ \hfill by lemma \ref{}}
  \prf{$\Gamma ; \Psi, x:A \vdash x:A $\hfill by rule}
  \prf{$\Gamma ; \Psi, x :A \vdash M~x : B$ \hfill by rule and $[x/x]B = B$}
  \prf{$\Gamma ; \Psi \vdash \lambda x.M~x : \Pityp x A B$\hfill by rule}
  \pcase{\ibnc{\Gamma ; \Psi, x{:}A \vdash M_1 : B}{\Gamma ; \Psi \vdash M_2 : A}{\Gamma ; \Psi \vdash (\lambda x.M_1)~M_2 \equiv [M_2/x]M_1 : [M_2/x]B}{}}
  \prf{$\Gamma ; \Psi, x{:}A \vdash M_1 : B$ \hfill by premise}
  \prf{$\Gamma ; \Psi \vdash \lambda x.M_1 : \Pityp x A B$ \hfill by rule}
  \prf{$\Gamma ; \Psi \vdash (\lambda x.M_1)~M_2 : [M_2/x]B$ \hfill by rule}
%  \prf{$\Gamma\vdash \Psi :\ctx$ \hfill by Lemma \ref{lm :fulllfctxwf}}
  \prf{$\Gamma ; \Psi \vdash [M_2/x]M_1 : [M_2/x]B$\hfill by Lemma \ref{}}
  \pcase{\ibnc{\Gamma ; \Phi \vdash N : A}{\Gamma ; \Psi \vdash \sigma : \Phi}{\Gamma ; \Psi \vdash \unbox{\Phi \vdash N}{\sigma} \equiv [\sigma]N : [\sigma]A}{}}
  \prf{$\Gamma \vdash [\sigma]N : [\sigma]A$ \hfill by Lemma \ref{}}
  \prf{$\Gamma; \Phi \vdash N : A$ \hfill by premise}
  \prf{$\Gamma\vdash \Phi \vdash N : \Phi \vdash A$ \hfill by rule}
  \prf{$\Gamma\vdash \cbox{\Phi \vdash N} : \cbox{\Phi \vdash A}$ \hfill by rule}
  \prf{$\Gamma ; \Psi \vdash \unbox{\Phi \vdash N}{\sigma}: [\sigma]A$ \hfill by rule}
  \pcase{\icnc{\Gamma \vdash \Psi \equiv \Phi: \tmctx}{
      \Gamma; \Psi \vdash A \equiv \tm : \lftype}{\Gamma; \Psi \vdash A \equiv B : \lftype}{\Gamma \vdash \Psi, x:A \equiv \Phi, x:B : \tmctx}{}}


  \prf{$\Gamma \vdash \Psi: \tmctx$ \hfill by IH}
  \prf{$\Gamma \vdash \Phi: \tmctx$ \hfill by IH}






\infer{\Gamma \vdash \Psi, x{:}A : \tmctx}
{\Gamma \vdash \Psi : \tmctx & \Gamma ; \Psi \vdash A : \lftype & \Gamma ; \Psi \vdash A \equiv \tm : \lftype}




\end{proof}

























\begin{lemma}
  Let $J = \{\}$
  If $\Gamma \vdash \Psi \equiv \Psi' : \ctx$ and $\Gamma;\Psi \vdash J$ then $\Gamma;\Psi' \vdash J $
  The symetry come from the symetry of the equivalence
\end{lemma}

\begin{proof}

We use the induction on
\end{proof}

%\begin{lemma}
 % If $\Gamma; \Psi \vdash M \equiv N : A $ and $\Gamma ; \Psi \vdash B:K$ then $\Gamma \vdash [M/x]$

%\end{lemma}













































\begin{lemma}
  If $\forall \Gamma' \leq_\rho \Gamma,t_1,t_2$ where $\Gamma' \vdash t_1 : \tau_1$ and $\Gamma' \vdash t_2 : \tau_1$\\
  $\Gamma' \Vdash t_1 = t_2 : \{\rho\}\tau_1 \Longrightarrow \Gamma' \Vdash \{\rho\}w~t_1 = \{\rho\}w'~t_2 : \{\rho, t_1/x\}\tau_2$  then $\Gamma \vdash w \equiv w' : (y : \tau_1)\arrow \tau_2$
\end{lemma}







%\begin{lemma}  \mbox{for all}~ \Gamma' \leq_\rho \Gamma,~t_1,~t_2 ~\mbox{where}~
%\Gamma' \vdash t_1 : \tau_1~\mbox{and}~
%\Gamma' \vdash t_2 : \tau_1~\\
%&&~\Gamma' \Vdash t_1 = t_2 : \{\rho\}\tau_1 \Longrightarrow \Gamma' \Vdash \{\rho\}w~t_1 = \{\rho\}w'~t_2 : \{\rho, t_1/x\}\tau_2

 % $\Gamma\vdash w \equiv w' : (y:\tau_1)\arrow \tau_2$
%\end{lemma}

%\begin{proof}
 % \mbox{for all}~ \Gamma' \leq_\rho \Gamma,~t_1,~t_2 ~\mbox{where}~
%\Gamma' \vdash t_1 : \tau_1~\mbox{and}~
%\Gamma' \vdash t_2 : \tau_1~\\
%&&~\Gamma' \Vdash t_1 = t_2 : \{\rho\}\tau_1 \Longrightarrow \Gamma' \Vdash \{\rho\}w~t_1 = \{\rho\}w'~t_2 : \{\rho, t_1/x\}\tau_2
%\end{proof}



\begin{proof}
  We have :  $\forall \Gamma' \leq_\rho \Gamma.~\Gamma' \vdash t_1 = t_2 : \{\rho\}\tau_1 \Longrightarrow \Gamma' \vdash \{\rho\}w~t_1 = \{\rho\}w'~t_2 : \{\rho, t_1/x\}\tau_2$\\
  Suppose that we have : $\Gamma' \vdash t_1 = t_2 : \{\rho\}\tau_1$.\\
  We have : $\Gamma' \vdash \{\rho\}w~t_1 = \{\rho\}w'~t_2 : \{\rho, t_1/x\}\tau_2$\\
 We have five possibilities :
\begin{itemize}
\item $w = w'$, $t_1 = t_2$ and $\infer{\Gamma'\vdash \{\rho\}w~t_1 = \{\rho\}w~t_1 : \{\rho, t_1/x\}\tau_2}{\Gamma'\vdash \{\rho\}w~t_1 : \{\rho, t_1/x\}\tau_2 }$ :\\
   By induction on the structure of the last rules, we have 2 possibilities :
    \begin{itemize}
    \item $\infer{\Gamma' \vdash \{\rho\}w~t_1 : \{\rho, t_1/y\}\tau_2}{\Gamma' \vdash \{\rho\}w: (y:\tau_1') \arrow \{\rho\}\tau_2 & \Gamma' \vdash s : \tau_1'}$:\\
      %%%%%%%%%%%%%%%HOW TO know that \{\rho\}tau1 equiv tau1'?????????????
      So we have :$ \Gamma' \vdash \{\rho\}w : (y :\tau_1')\arrow \{\rho\}\tau_2$

    \item $\infer{\Gamma' \vdash \{\rho\}w~t_1 : \{\rho, t_1/y\}\tau_2}{\Gamma' \vdash \{\rho\}w~t_1 : \tau' & \Gamma' \vdash \tau' \equiv \{t_1/y\}\tau_2}$ : \\
      By induction, we have : $\Gamma' \vdash \{\rho\}w $
    \end{itemize}
    So we have : $\infer{\Gamma' \vdash \{\rho\}w \equiv \{\rho\}w : (y :\tau_1')\arrow \{\rho\}\tau_2}{\Gamma' \vdash \{\rho\}w : (y :\tau_1')\arrow \{\rho\}\tau_2}$

 \item $\infer{\Gamma\vdash t'\equiv t :\tau}{\Gamma\vdash t\equiv t' :\tau}$
 \item $\infer{\Gamma\vdash t_1\equiv t_3 : \tau}{\Gamma \vdash t_1 \equiv t_2 : \tau & \Gamma \vdash t_2 \equiv t_3 :\tau}$
 \end{itemize}
\end{proof}


==> compsub.tex <==




\begin{corollary}[Extension of substitution]
  \label{lm:lemaux2}
Let $y$ be a new name s.t. $y \notin dom(\Gamma')$ and $y \notin dom(\Gamma)$.  
If $\Gamma' \vdash \theta : \Gamma$ and $\Gamma' \vdash \{\theta\}\tau$ then 
   $\Gamma', y : \{\theta\}\tau, \Gamma' \vdash \theta,y/y :  \Gamma, y :\tau $
\end{corollary}
\LONGVERSION{
\begin{proof}~\\% [1em]
  \prf{$\Gamma', y:\{\theta\}\tau \vdash \theta : \Gamma$ \hfill by Lemma \ref{lm:wkwksub} }
  \prf{$\vdash \Gamma, y:\{\theta\}\tau$ \hfill by Lemma \ref{lm:ctxwf}}
  \prf{$\Gamma, y:\{\theta\}\tau \vdash y:\{\theta\}\tau $ \hfill by Lemma \ref{}}
\prf{$\Gamma', y:\{\theta\}\tau \vdash \theta, y/ y :\Gamma, y: \tau$ \hfill by rule}
\end{proof}
}

\medskip


\begin{lemma}[Computation Substitution (Simultaneous)]~
  \begin{enumerate}
  \item If $\Gamma' \vdash \theta : \Gamma$ and $\Gamma; \Psi \vdash \JLF$ then $\Gamma' ; \{\theta\}\Psi \vdash \{\theta\}\JLF$.
  \item If $\Gamma' \vdash \theta : \Gamma$ and $\Gamma \vdash \Jcomp$ then $\Gamma' \vdash \{\theta\}\Jcomp$.
  \end{enumerate}  
\end{lemma}
\begin{proof}
\pcase{$\ibnc{x{:} \tau \in \Gamma}{\vdash \Gamma}{\Gamma \vdash x : \tau}{}$}
\prf{$\Gamma' \vdash \theta : \Gamma$ \hfill by assumption}
\prf{$\Gamma' \vdash \theta_0, y/x : \Gamma_0, x{:}\tau$ and $\theta = \theta_0,y/x \theta_1$ and $\Gamma = \Gamma_0, x{:}\tau, \Gamma_1$ \hfill by inversion}
\prf{$\Gamma' \vdash t : \{\theta_0\}\tau$ \hfill by inversion}
\prf{$\Gamma' \vdash t : \{\theta\}\tau$ \hfill since $\tau$ does not depend on the variable in $(x{:}\tau,\Gamma_1)$}
\prf{$\Gamma' \vdash \{\theta\}x : \{\theta\}\tau$ \hfill since $\{\theta\}x = t$ and $t$ does not depend on the variable in $(x{:}\tau,\Gamma_1)$}



\pcase{$\ibnc{\Gamma \vdash t : (y:\tau_1) \arrow \tau_2 }
              {\Gamma \vdash s : \tau_1}
              {\Gamma \vdash t~s : \{s/y\}\tau_2}{}
$}
\prf{$\Gamma' \vdash \{\theta\}s : \{\theta\}\tau_1$ \hfill by IH}
\prf{$\Gamma' \vdash \{\theta\}t : \{\theta\}((y:\tau_1) \arrow \tau_2)$ \hfill by IH}
\prf{$\Gamma' \vdash \{\theta\}t : (y: \{\theta\}\tau_1) \arrow \{\theta,y/y\}\tau_2$ \hfill by subst. definition}
\prf{$\Gamma' \vdash (\{\theta\} t)~(\{\theta\}s) : \{\{\theta\}s/y\}(\{\theta,y/y\}\tau_2)$ \hfill by rule}
\prf{$\Gamma' \vdash \{\theta\}(t~s) : \{\{\theta\}s/y\}(\{\theta,y/y\}\tau_2)$ \hfill by subst. definition}
\prf{$\Gamma' \vdash \{\theta\}(t~s) :\{\theta\}(\{s/y\}\tau_2)$ \hfill by compositionality of substitution}

\pcase{$\ianc{\Gamma, y:\tau_1 \vdash t : \tau_2}
             {\Gamma \vdash \tmfn y t : (y:\tau_1) \arrow \tau_2}{}$}
\prf{$\Gamma' \vdash \theta : \Gamma$ \hfill by assumption}
\prf{$\vdash \Gamma, y :\tau_1$ \hfill by Lemma \ref{lm:ctxwf}}
\prf{$\Gamma \vdash \tau_1$ \hfill by inversion}
\prf{$\Gamma\vdash\{\theta\}\tau_1$ \hfill by IH}
\prf{$\Gamma', y : \{\theta\}\tau_1\vdash_w \theta, y/y : \Gamma, y:\tau_1$ \hfill by Lemma \ref{lm:lemaux2}}
\prf{$\Gamma', y:\{\theta\}\tau_1 \vdash \{\theta,y/y\}t : \{\theta,y/y\}\tau_2$ \hfill by IH}
\prf{$\Gamma' \vdash \tmfn y {\{\theta,y/y\}t} : (y:\{\theta\}\tau_1) \arrow \{\theta,y/y\}\tau_2$ \hfill by rule}
\prf{$\Gamma' \vdash \{\theta\}(\tmfn y t) : \{\theta\}((y:\tau_1) \arrow \tau_2)$ \hfill by subst. definition}

\pcase{\ianc{ \Gamma, \psi:\cbox{\tmctx}, p:\cbox{~\unboxc{\psi} \vdash_\# \tm}  \vdash t_v : \{p / y\}\tau}{\Gamma \vdash ({\psi,p \mto t_v}) : \IH } where $\IH = (\psi : \cbox{\tmctx}) \arrow (y:\cbox{\psi \vdash \tm}) \arrow \tau$}
\prf{$\Gamma'\vdash \theta : \Gamma$ \hfill by assumption}
\prf{$\vdash \Gamma, \psi:\cbox{\tmctx}, p:\cbox{~\unboxc{\psi} \vdash_\# \tm}$\hfill by Lemma \ref{lm:ctxwf}}
\prf{$\vdash \Gamma, \psi:\cbox{\tmctx}$\hfill by inversion}
\prf{$\Gamma, \psi:\cbox{\tmctx} \vdash \cbox{~\unboxc{\psi} \vdash_\# \tm}$\hfill by inversion}
\prf{$\Gamma\vdash \psi:\cbox{\tmctx}$\hfill by inversion}
\prf{$\Gamma'\vdash \cbox{\tmctx}$\hfill by IH and definition of substitution}
\prf{$\Gamma',\psi:\cbox{\tmctx} \vdash \theta, \psi/\psi : \Gamma, \psi:\cbox{\tmctx}$ \hfill by Lemma \ref{lm:lemaux2} and since $\psi$ is free}
\prf{$\Gamma', \psi:\cbox{\tmctx} \vdash \cbox{~\unboxc{\psi} \vdash_\# \tm}$\hfill by IH}
\prf{$\Gamma',\psi:\cbox{\tmctx}, p : \cbox{~\unboxc{\psi} \vdash_\# \t} \vdash \theta, \psi/\psi, p/p : \Gamma, \psi:\cbox{\tmctx}, p:  \cbox{~\unboxc{\psi} \vdash_\# \t}$ \hfill by Lemma \ref{lm:lemaux2} and since $\psi$ is free}
\prf{$\Gamma', \psi:\cbox{\tmctx}, p:\cbox{~\unboxc{\psi} \vdash_\# \tm}  \vdash \{\theta\} t_v : \{\theta, p / y\}\tau$ \hfill by IH and by definition of substitution}
\prf{$\Gamma' \vdash \{\theta\} ({\psi,p \mto t_v}) : \{\theta\}\IH$ \hfill by rule and by definition of substitution}
\end{proof}


==> injecappl.tex <==
\begin{lemma}
  \label{lm : equivctx}
  If $\Gamma \vdash \tau_1 \equiv \tau_1' : ?$ and $\Gamma, y:\tau_1 \vdash \tau_2 \equiv \tau_2'$
  then $\Gamma, y :\tau_1' \vdash \tau_2 \equiv \tau_2'$
\end{lemma}



\begin{proof}
  \prf{$\Gamma\vdash \tau_1' : ?$ \hfill by Lemma \ref{}}
  \prf{$\vdash \Gamma$ \hfill by Lemma}
  \prf{$\vdash\Gamma, y:\tau_1'$ \hfill by  definition of well-formed computation context}
  \prf{$\Gamma, y :\tau_1' \vdash_w \rho : \Gamma$ \hfill by Lemma \ref{}}
  \prf{$\Gamma, y :\tau_1' \vdash \rho : \Gamma$ \hfill by Lemma \ref{}}
  \prf{$\Gamma,y:\tau_1'\vdash y:\tau_1'$\hfill by rule}
  \prf{$\Gamma, y:\tau_1' \vdash y : \tau_1$\hfill by rule}
  \prf{$\Gamma, y:\tau_1' \vdash \rho, y/y : \Gamma, y:\tau_1'$ \hfill by construction of computation substitution}
    \prf{$\Gamma, y:\tau_1'\vdash \tau_2\equiv \tau_2 $ \hfill by Lemma \ref{}}
\end{proof}




\begin{theorem}[Function Type Injectivity]
  \begin{enumerate}
  \item
    If $\Gamma \vdash (y:\tau_1) \arrow \tau_2 : u $
    then
    $\Gamma \vdash \tau_1 $ and
    $\Gamma, y:\tau_1 \vdash \tau_2$.
  \item If $\Gamma \vdash (y:\tau_1) \arrow \tau_2 \equiv (y:\tau'_1) \arrow\tau'_2 $
    then
    $\Gamma \vdash \tau_1 \equiv \tau'_1$ and
    $\Gamma, y:\tau_1 \vdash \tau_2 \equiv \tau'_2$.
  \end{enumerate}
\end{theorem}

\begin{proof}
  \begin{enumerate}
  \item
    \pcase{\ianc{\Gamma, y: \tau_1\vdash \tau_2}{\Gamma\vdash (y:\tau_1)\arrow \tau_2}{}}
    \prf{$\Gamma, y: \tau_1\vdash \tau_2$ \hfill by assumption}
    \prf{$\vdash \Gamma, y: \tau_1$ \hfill by Lemma \ref{}}
    \prf{$\Gamma \vdash \tau_1$ \hfill by definition}
  \item
    By induction on the derivation.\\
    \pcase{\ianc{\Gamma \vdash (y:\tau_1) \arrow \tau_2}{\Gamma \vdash (y:\tau_1) \arrow \tau_2 \equiv(y:\tau_1) \arrow \tau_2}{}}
    \prf{$\Gamma \vdash\tau_1$ and $\Gamma, y:\tau_1 \vdash \tau_2$ \hfill by 1.}
    \prf{$\Gamma \vdash \tau_1 \equiv \tau_1$ \hfill by rule}
    \prf{$\Gamma, y:\tau_1 \vdash \tau_2 \equiv \tau_2 $ \hfill by rule}
    %
    \pcase{\ianc{\Gamma \vdash (y: \tau_1') \arrow \tau_2'\equiv (y:\tau_1) \arrow \tau_2}{\Gamma \vdash (y:\tau_1) \arrow \tau_2 \equiv (y:\tau'_1) \arrow\tau'_2 }{}}
    \prf{$\Gamma\vdash (y: \tau_1') \arrow \tau_2'\equiv (y:\tau_1) \arrow \tau_2$ \hfill by assumption}
    \prf{$\Gamma \vdash \tau_1' \equiv \tau_1$ by IH}
    \prf{$\Gamma \vdash \tau_1 \equiv \tau_1'$ by rule}
    \prf{$\Gamma, y:\tau_1' \vdash \tau_2' \equiv \tau_2$. by IH}
    \prf{$\Gamma, y:\tau_1' \vdash \tau_2 \equiv \tau_2'$. by rule}
    \prf{$\Gamma, y:\tau_1 \vdash \tau_2 \equiv \tau_2'$ \hfill by Lemma \ref{lm : equivctx}}
    %
    \pcase{\ibnc{\Gamma \vdash (y:\tau_1)\arrow \tau_2 \equiv (y:\tau_1'') \arrow \tau_2''}{\Gamma \vdash (y:\tau_1'')\arrow \tau_2'' \equiv (y:\tau_1') \arrow \tau_2'}{\Gamma \vdash (y:\tau_1)\arrow \tau_2 \equiv (y:\tau_1') \arrow \tau_2'}{}}
    \prf{$\Gamma \vdash \tau_1\equiv \tau_1''$ \hfill by IH}
    \prf{$\Gamma \vdash \tau_1''\equiv \tau_1'$ \hfill by IH}
    \prf{$\Gamma \vdash \tau_1\equiv \tau_1'$ \hfill by rule}
    \prf{$\Gamma, y : \tau_1 \vdash \tau_2\equiv \tau_2''$ \hfill by IH}
    \prf{$\Gamma, y : \tau_1'' \vdash \tau_2\equiv \tau_2''$ \hfill by Lemma \ref{lm : equivctx}}
    \prf{$\Gamma, y : \tau_1'' \vdash \tau_2''\equiv \tau_2'$ \hfill by IH}
    \prf{$\Gamma, y : \tau_1'' \vdash \tau_2\equiv \tau_2'$ \hfill by rule}
    \prf{$\Gamma, y : \tau_1 \vdash \tau_2\equiv \tau_2'$ \hfill by Lemma \ref{lm : equivctx}}
    %
    \pcase{\ibnc{\Gamma \vdash \tau_1 \equiv \tau_1'}{\Gamma, y:\tau_1 \vdash \tau_2\equiv \tau_2'}{\Gamma \vdash (y:\tau_1)\arrow \tau_2 \equiv (y:\tau_1') \arrow \tau_2'}{}}
  \end{enumerate}
\end{proof}


==> proof.tex <==
\section{Proof}



 \subsection{Completness}


%\begin{theorem}
 % \begin{enumerate}
  %\item If $\Gamma \vdash t : \tau$ then $\Gamma \vdash \tau$.
  %\item If $\Gamma \vdash t \equiv t' : \tau$ then $\Gamma \vdash t : \tau$ and
  %  $\Gamma \vdash t' : \tau$.
%  \end{enumerate}
%\end{theorem}

%\begin{proof}
%  \begin{enumerate}
%  \item
%    By induction on the structure of the rules.\\
    %We will only interest on the
%  \item $\infer{\Gamma \vdash y : \tau}{y:\tau \in \Gamma&\vdash\Gamma}$\\
%    So by construction of $\vdash \Gamma$, we have : $\Gamma = \Gamma', \Gamma''$ and $\Gamma' \vdash \tau$.\\
%    $\Gamma' = x_1 : \tau_1, ..., x_n : \tau_n$\\
%    With $\Gamma \vdash x_1/x_1,...,x_n/x_n : \Gamma'$, we have $\Gamma\vdash \{x_1/x_1,...,x_n/x_n\}\tau$.\\
%    So we have the result : $\Gamma\vdash\tau$.\\
%  \item $\infer{\Gamma \vdash t~s : \{s/y\}\tau_2}{\Gamma \vdash t : (y:\tau_1) \arrow \tau_2 & \Gamma \vdash s : \tau_1}$
%    So by induction hypothesis, we have : $\Gamma \vdash (y:\tau_1) \arrow \tau_2$ and $\Gamma \vdash \tau_1$




%\item
%  $\infer{\Gamma \vdash \tmfn y t : (y:\tau_1) \arrow \tau_2}{\Gamma, y:\tau_1 \vdash t : \tau_2 & \Gamma \vdash \tau_1}$
%  By induction hypothesis, we have :\\
%      $\infer{\Gamma\vdash (y : \tau_1) \arrow \tau_2}{\Gamma \vdash \tau_1 & \Gamma, y:\tau_1 \vdash \tau_2}$
%\item
%\infer{\Gamma \vdash t : \tau}
%{\Gamma \vdash t : \tau' & \Gamma \vdash \tau' \equiv \tau}
%\item
%\infer{\Gamma \vdash [C] : [T]}{\Gamma \vdash C : T}

%\infer{\Gamma \vdash \tmrec {\psi.y.\tau} {t_v} {t_{\mathsf{app}}} {t_{\clam}} t : \{\Psi/\psi, t/y\}\tau}
%{
%  \begin{array}{l@{~}l@{~}l}
%\Gamma & \vdash & t : [\Psi \vdash \tm]\\[0.5em]
%\Gamma, \phi:\tmctx, m:[\phi, x:\tm \vdash \tm], f_m:\{(\phi, x:\tm)/\psi, m /y \} \tau & \vdash & t_{\clam} : \{\phi/\psi, [\phi \vdash \clam~\lambda x.m[\id_\phi, x] / y\}\tau\\[0.5em]
%\Gamma, \psi:\tmctx, m:[\psi \vdash \tm], n:[\psi \vdash \tm], f_m: \{m/y\}\tau, f_n: \{n/y\}\tau & \vdash & t_{\mathsf{app}} : \{[\psi \vdash\capp~m[\id_\psi]~n[\id_\psi]]/y\}\tau
%\\[0.5em]
% \Gamma, \psi:\tmctx, p:\#[\psi \vdash \tm] & \vdash & t_v : \{p / y\}\tau

%  \end{array}
%}

 % \item
  %  By induction on the structure of the rules.\\
  %\end{enumerate}
%\end{proof}




\begin{theorem}[Completeness]\label{lem:SemComplete}
If $\Gamma \Vdash t = t' : \tau$ then $\Gamma \vdash t : \tau$ and
$\Gamma \vdash t' : \tau$ and
$\Gamma \vdash t \equiv t' : \tau$ and
$\Gamma \vdash \tau$.
\end{theorem}




 \input{completness.tex}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> related.tex <==
\section{Type Theory and Higher-Order Abstract Syntax -- A Retrospective }
Before we describe \cocon in more detail, we first take a look back at
the fundamental challenges that we face when combining HOAS
representations with dependent types and then survey the results upon
which \cocon is built.

 \subsection{Intensional and Extensional Functions -- A World of a Difference }
To understand the fundamental difference between defining HOAS trees in LF vs.
defining HOAS-style trees using inductive types, let us consider an inductive type
\lstinline!D! with one constructor
\lstinline!abs: (D -> D) -> D!. What is the problem with such a
definition in type theory? -- In functional ML-like languages, this is, of course,
possible. However, the function argument to the constructor \lstinline!abs! is
opaque and we would not be able to pattern match deeper on the
argument to inspect the shape and structure of the syntax
tree that is described by it. We can only observe it by applying it to
some argument. The resulting encoding also would not be adequate,
i.e.~there are terms of type \lstinline!D! that are in normal form but
do not uniquely correspond to a term in the object language we try to
model. As a consequence, we may need to rule out such ``exotic''
representation \cite{Despeyroux:TLCA95}. But there is a more fundamental problem. In proof
assistants based on type theory such as Coq or Agda, we cannot afford
to work within an inconsistent system and we demand that all programs we write are
terminating. The definition of a constructor \lstinline!abs! as given
previously would be forbidden as it violates what is known as the
positivity restriction. Were we to allow it, we can easily write
non-terminating programs -- even without making a recursive call.

% data D : u where
% inj : (D -> D) -> D
\noindent
\begin{minipage}{4cm}
\begin{lstlisting}
out : D -> (D -> D)
out  (abs f) = f
\end{lstlisting}
\end{minipage}
\begin{minipage}{5cm}
\begin{lstlisting}
omega : D
omega = abs (\x -> (out x) x)
\end{lstlisting}
\end{minipage}
\begin{minipage}{6cm}
\begin{lstlisting}
Omega : D
Omega = (out omega) omega
\end{lstlisting}
\end{minipage}



Here we simply write two functions: the function \lstinline!out! unpacks an
object of type \lstinline!D! using pattern matching and the function
\lstinline!omega! creates an object of type \lstinline!D!. Using
\lstinline!out! and \lstinline!omega! we can now write a
non-terminating program that will continue to reproduce itself.

This example begs two questions: How can we reason inductively about
LF definitions if they are seemingly not inductive? Do we have to
simply give up on HOAS definitions to model syntactic structures
within type theory to remain consistent?

% \subsection{Higher-Order Abstract Syntax in Dependent Type Theories}

% \subsection{Logical Framework Tradition}
% % INCORPORATED INTO INTRODUCTION 
% % There has been a lot of work in trying to make HOAS work in a
% % dependently type proof language \cite{Despeyroux:LPAR94,Felty12,Chlipala:ICFP08}
% % This line of work has the issue of exotic terms and it only inherits
% % alpha-renaming from the meta-language, but not substitution; it also
% % does not scale beyond second order representations.
% %
% %
% Two decades ago \citet{Despeyroux97} made
% the key observation that we can mediate between the weak LF function and the strong
% computation-level function space using a box-modality. The authors
% describe a simply typed lambda-calculus with iteration and case
% constructs which preserves the adequacy of higher-order abstract
% syntax encodings. The well-known paradoxes are avoided through the use
% of a modal box operator which obeys the laws of S4. In addition to
% being simply typed, all computation had to be on closed HOAS trees. \citet{Despeyroux99}
% sketched an extension of this line of work to dependent type theory --
% however it lacks a normalization proof.
% % does not have a hierarchy of universes

% \beluga took another important step towards writing inductive proofs
% about HOAS trees by generalizing the box-modality to a contextual
% modal type \cite{Nanevski:ICML05}. This allows us to
% characterize HOAS tress that depend on a context of
% assumptions. Moreover, we can analyze these contextual HOAS trees using case
% analysis and recursion. However, in \beluga, we treat
% syntactic representation of contextual HOAS trees as data and write
% recursive programs about it hence segregating data from
% computation. The resulting language is an indexed type system in the
% tradition of \citet{Zenger:TCS97} and \citet{Xi99popl}. This is evident
% in the normalization proof of \beluga which takes advantage of the
% modularity in its design.

% Building on this line of work, \cocon takes the next step and extends
% existing frameworks to a dependent type theory with recursion and
% universes. In particular, we do not strictly separate data from
% computation, but allow computations to be embedded into data. This
% finally allows us to combine the world of type theory and logical
% frameworks inheriting the best of both worlds.

% \subsection{Metaprogramming and Dependent Types -- [moved to future
% work / conclusion -bp}
% One might also wonder whether we actually need the ability to define
% HOAS definitions in a type theory -- after all, we can always model
% binding structures via well-scoped de Bruijn representations. However,
% building up such infrastructure consistently






% Traditionally, implementing HOAS in systems without a specification
% framework is troublesome because of the positivity restriction for
% inductive types. To overcome this problem, weaker forms of HOAS use an
% abstract type to represent variables and obtain a strictly positive
% type. Examples of this aret the work of~\citet{Chlipala:ICFP08}
% and~\citet{Despeyroux:1994:HAS:645708.664171}. Weaker forms of HOAS
% are convenient but they do not get substitution from $\beta$-reduction
% in the host language and make complicated to deal with open terms.

% Another option is to implement binders using de~Bruijn indices. A
% convenient way is using well-scoped de~Bruijn
% indices~\cite{Benton:JAR12}, where substitution is implemented as an
% inductive data type and its structural properties need to be proved
% manually. There are implementations of de~Bruijn indices that provide
% and facilitate proving the required lemmas. One example is
% Autosubst~\cite{Schaefer2015} that implements a decision procedure to
% compare terms with explicit substitutions. The Nameless
% Painless~\cite{Pouillard:2011} approach is based on de~Bruijn indices,
% but it simplifies the arithmetic reasoning by hiding the numbers in an
% abstract ``world'' representation. Finally, GMeta~\cite{Lee2012}
% simplifies implementing first-order binding representations (e.g.:
% de~Bruijn indices) using generic programming to provide proofs for the lemmas
% about binders.
% % \inlinetodo{Consider DBLib by
% %   Fran\c{c}ois Pottier, but there is no publication associated with
% %   the library}

% More recently, ~\citet{Allais:2017} propose a way of encoding syntax
% (as opposed to syntax and judgments) in Agda using a generic type and
% scope preserving semantics. This allows them to prove lemmas about the
% semantics and then reuse them to implement renaming, substitution,
% normalization by evaluation and CPS transformations.

% % Finally, a possible approach is to use nominal logic~\cite{Pitts:2003}
% % that uses an infinite set of atoms (abstract names) to replace the
% % position based approach. These ideas have been implemented in
% % Nominal~\cite{Urban:JAR08} package of
% % Isabelle~\cite{Nipkow-Paulson-Wenzel:2002} however it is not currently
% % clear how to implement these ideas in a dependently typed system.

% Finally, thanks to its specification framework, Cocon is
% well-positioned to implement meta-programming in dependently typed
% systems where syntax can be reflected into LF objects where
% computational functions can manipulate them. There is interest in
% doing this in existing systems as a way of implementing tactics and
% elaboration, for example the MTAC~\cite{ziliani:2015} system for Coq,
% or elaboration reflection~\cite{Christiansen:PHD} for Idris implement
% meta-programming (The Agda proof assistant also implements Idris-style
% reflection). What Cocon offers to meta-programming is the ability of
% processing structures with binders in a type safe and convenient way,
% instead, for example, of the de~Bruijn representation that the Idris
% reflection offers.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sconversion.tex <==
\section{Proof of Semantic Type Conversion}
\begin{lemma}
  Let $\Gamma = x_1 : \tau_1,...,x_n : \tau_n, \Gamma'$\\
  If $\vdash\Gamma$ then $\Gamma \vdash x_1/x_1,...,x_n/x_n :  x_1 : \tau_1,...,x_n : \tau_n$
\end{lemma}

\begin{proof}
  By recurrence on $n$.\\
  \pcase{$n = 0$}
  \prf{$\vdash \Gamma$ \hfill by assumption}
  \prf{$\Gamma \vdash \cdot : \Gamma$\hfill by rule}
  %
  \pcase{It is prove for $m = n-1$}
  \prf{$\Gamma \vdash x_1/x_1,...,x_m/x_m :  x_1 : \tau_1,...,x_m : \tau_m$ \hfill by RH}
  \prf{$x_{m+1}\notin dom(x_1/x_1,...,x_m/x_m)$ \hfill by def. of $\vdash\Gamma$}
  \prf{$x_{m+1} : \tau_{m+1} \in \Gamma$ \hfill by definition}
  \prf{$\Gamma\vdash  x_1/x_1,...,x_m/x_m, x_{m+1}/x_{m+1} :  x_1 : \tau_1,...,x_m : \tau_m, x_{m+1} : \tau_{m+1}$ \hfill by rule}
\end{proof}


\begin{lemma}
  \label{lm:semeqtosyntype}
  If $\Gamma \Vdash \tau = \tau'$ then
  \begin{enumerate}
  \item $\Gamma \vdash \tau'$
  \item $\Gamma \vdash \tau$
  \end{enumerate}
\end{lemma}

\begin{proof}
  \begin{enumerate}
  \item  By definition of $\Gamma \vdash \tau_1 \whnf \tau_2$
  \item TODO
  \end{enumerate}
\end{proof}

\begin{lemma}
  \label{lm : semsyntypeq}
  If $\Gamma \Vdash \tau = \tau' $ then $\Gamma \vdash \tau \equiv \tau'$
\end{lemma}


\begin{proof}
  By induction on $\Gamma\Vdash \tau$.\\
  \pcase{$\Gamma\Vdash \cbox{T_1}\equiv \cbox{T_2}$}
  \prf{$\Gamma \vdash T_1 \equiv T_3$ \hfill by definition}
  \prf{$\Gamma \vdash \cbox{T_1} \equiv \cbox{T_3}$ \hfill by rule}
  \prf{$\Gamma \vdash \cbox{T_2} \equiv \cbox{T_3}$ \hfill by definition}
  \prf{$\Gamma \vdash \cbox{T_1} \equiv \cbox{T_2}$ \hfill by symetry and transitivity closure of the equivalence}
  %
  \pcase{$\Gamma \Vdash (y:\tau_1) \arrow \tau_2 = (y : \tau_1') \arrow \tau_2'$}
  \prf{$\Gamma \vdash (y:\tau_1')\arrow \tau_2' \whnf (y :\tau_1'' )\arrow \tau_2'' $ \hfill by assumption}
  \prf{$\Gamma \vdash (y:\tau_1')\arrow \tau_2' \equiv (y :\tau_1'' )\arrow \tau_2'' $ \hfill by definition}
  \prf{$\forall \Gamma' \leq_\rho \Gamma.\Gamma'\Vdash \{\rho\}\tau_1 = \{\rho\} \tau_1'')$\hfill by assumption}
  \prf{$\Gamma\Vdash \tau_1 =\tau_1''$ \hfill since taken $\Gamma = \Gamma'$ and $\rho$ the identity}
  \prf{$\Gamma \vdash \tau_1''$ \hfill by Lemma \ref{lm:semeqtosyntype}}
  \prf{$y\notin dom(\Gamma)$ \hfill by construction}
  \prf{$\vdash \Gamma$ \hfill by Lemma \ref{}}
  \prf{$\vdash \Gamma, y:\tau_1''$ \hfill by rule}
  \prf{$\Gamma, y : \tau_1'' \leq_\rho \Gamma$ \hfill by Lemma \ref{} and $\rho$ is the identity}
  \prf{$\Gamma, y : \tau_1'' \vdash y : \tau_1''$ \hfill by rule}
  \prf{$\neut y$ \hfill by def.}
  \prf{$\Gamma, y : \tau_1'' \Vdash y :\tau_1''$ \hfill by Lemma \ref{}}
  \prf{$\forall \Gamma'\leq_\rho \Gamma. \Gamma' \Vdash t : \{\rho\}\tau_1 \Longrightarrow \Gamma' \Vdash \{\rho, t/y\} \tau_2 = \{\rho,t/y\}\tau_2'' $ \hfill by assumption}
  \prf{$\Gamma, y:\tau_1'' \Vdash \tau_2 = \tau_2''$ \hfill since taking $\Gamma' = \Gamma, y:\tau_1''$ and $\rho$ the identity for the variable of $\Gamma$} %%%% not total sure !
  \prf{$\Gamma \vdash \tau_1 = \tau_1''$ \hfill by IH}
  \prf{$\Gamma, y : \tau_1''\vdash \tau_2 = \tau_2''$ \hfill by IH}
  \prf{$\Gamma \vdash (y:\tau_1) \arrow \tau_2 \equiv (y: \tau_1'') \arrow \tau_2''$ \hfill by rules}
  \prf{$\Gamma \vdash (y:\tau_1) \arrow \tau_2 \equiv (y: \tau_1') \arrow \tau_2'$ \hfill by rules}
\end{proof}


\begin{theorem}
  \begin{enumerate}
    \item If $\Gamma \vdash (y:\tau_1) \arrow \tau_2 \equiv (y:\tau'_1) \arrow\tau'_2 $
      then $\Gamma \vdash \tau_1 \equiv \tau'_1$
    \item If $\Gamma \vdash (y:\tau_1) \arrow \tau_2 \equiv (y:\tau'_1) \arrow\tau'_2 $ and $\Gamma \vdash t : \tau_1$
      then $\Gamma \vdash \{t/y\}\tau_2 \equiv \{t/y\}\tau'_2$.
  \end{enumerate}
\end{theorem}

\begin{proof}
  By induction on the derivation.\\
  \begin{enumerate}
  \item
    By induction on the derivation.\\
    \pcase{\ianc{\Gamma \vdash (y:\tau_1) \arrow \tau_2}{\Gamma \vdash (y:\tau_1) \arrow \tau_2 \equiv(y:\tau_1) \arrow \tau_2}{}}
    \prf{$\Gamma \vdash\tau_1$ \hfill by inversion}
    \prf{$\Gamma \vdash \tau_1 \equiv \tau_1$ \hfill by rule}
    %
    \pcase{\ianc{\Gamma \vdash (y: \tau_1') \arrow \tau_2'\equiv (y:\tau_1) \arrow \tau_2}{\Gamma \vdash (y:\tau_1) \arrow \tau_2 \equiv (y:\tau'_1) \arrow\tau'_2 }{}}
    \prf{$\Gamma \vdash \tau_1' \equiv \tau_1$ by IH}
    \prf{$\Gamma \vdash \tau_1 \equiv \tau_1'$ by rule}
    %
    \pcase{\ibnc{\Gamma \vdash (y:\tau_1)\arrow \tau_2 \equiv (y:\tau_1'') \arrow \tau_2''}{\Gamma \vdash (y:\tau_1'')\arrow \tau_2'' \equiv (y:\tau_1') \arrow \tau_2'}{\Gamma \vdash (y:\tau_1)\arrow \tau_2 \equiv (y:\tau_1') \arrow \tau_2'}{}}
    \prf{$\Gamma \vdash \tau_1\equiv \tau_1''$ \hfill by IH}
    \prf{$\Gamma \vdash \tau_1''\equiv \tau_1'$ \hfill by IH}
    \prf{$\Gamma\vdash \tau_1 \equiv \tau_1'$\hfill by rule}
    %
    \pcase{\ibnc{\Gamma \vdash \tau_1 \equiv \tau_1'}{\Gamma, y:\tau_1 \vdash \tau_2\equiv \tau_2'}{\Gamma \vdash (y:\tau_1)\arrow \tau_2 \equiv (y:\tau_1') \arrow \tau_2'}{}}
  \item
    \pcase{\ianc{\Gamma \vdash (y:\tau_1) \arrow \tau_2}{\Gamma \vdash (y:\tau_1) \arrow \tau_2 \equiv(y:\tau_1) \arrow \tau_2}{}}
    \prf{$\Gamma, y:\tau_1 \vdash \tau_2$ \hfill by inversion}
    \prf{$\Gamma, y:\tau_1 \vdash \tau_2 \equiv \tau_2 $ \hfill by rule}
    \prf{$\Gamma \vdash \{t/y\}\tau_2 \equiv \{t/y\}\tau_2$ \hfill by Lemma \ref{}}
    %
    \pcase{\ianc{\Gamma \vdash (y: \tau_1') \arrow \tau_2'\equiv (y:\tau_1) \arrow \tau_2}{\Gamma \vdash (y:\tau_1) \arrow \tau_2 \equiv (y:\tau'_1) \arrow\tau'_2 }{}}
    \prf{$\Gamma \vdash t : \tau_1'$ \hfill by rule and 1.}
    \prf{$\Gamma \vdash \{t/y\} \tau_2' \equiv \{t/y\}\tau_2$\hfill by IH}
    \prf{$\Gamma \vdash \{t/y\} \tau_2 \equiv \{t/y\}\tau_2'$\hfill by rule}
    %
    \pcase{\ibnc{\Gamma \vdash (y:\tau_1)\arrow \tau_2 \equiv (y:\tau_1'') \arrow \tau_2''}{\Gamma \vdash (y:\tau_1'')\arrow \tau_2'' \equiv (y:\tau_1') \arrow \tau_2'}{\Gamma \vdash (y:\tau_1)\arrow \tau_2 \equiv (y:\tau_1') \arrow \tau_2'}{}}
    \prf{$\Gamma, \vdash \{t/y\}\tau_2\equiv \{t/y\}\tau_2''$ \hfill by IH}
    \prf{$\Gamma \vdash \tau_1\equiv \tau_1''$ \hfill by 1.}
    \prf{$\Gamma \vdash t : \tau_1''$ \hfill by rule}
    \prf{$\Gamma \vdash \{t/y\}\tau_2''\equiv \{t/y\}\tau_2'$ \hfill by IH}
    \prf{$\Gamma \vdash \{t/y\}\tau_2 \equiv \{t/y\}\tau_2'$ \hfill by rule}
    %
    \pcase{\ibnc{\Gamma \vdash \tau_1 \equiv \tau_1'}{\Gamma, y:\tau_1 \vdash \tau_2\equiv \tau_2'}{\Gamma \vdash (y:\tau_1)\arrow \tau_2 \equiv (y:\tau_1') \arrow \tau_2'}{}}
    \prf{$\Gamma \vdash \{t/y\} \tau_2\equiv \{t/y\}\tau_2'$ \hfill by Lemma \ref{}}
  \end{enumerate}
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{lemma}
  \begin{enumerate}
  \item If $\Gamma\vdash \Psi : \ctx$ and $\Psi = \Psi', \Psi''$ then $\Gamma; \Psi \vdash \sigma : \Psi'$
  \item If $\Gamma \vdash \Psi, x {:}A  \equiv \Phi, x {:} B : \ctx$ then $\Gamma; \Psi, x{:} A \vdash\sigma : \Phi, x {:}B$
  \item If $\Gamma\vdash \Psi \equiv \Phi: \ctx$ then $\Gamma; \Psi \vdash \sigma : \Phi$ and $\Gamma; \Phi \vdash \sigma' : \Psi$
  \end{enumerate}
\end{lemma}


\begin{proof}
  \begin{enumerate}
  \item  By induction on $\Psi'$.\\
    \pcase{$\Psi'= \cdot$}
    \prf{$\Gamma\vdash \Psi : \ctx$ \hfill by assumption}
    \prf{$\Gamma; \Psi \vdash \cdot : \cdot$ \hfill by rule}
    \pcase{$\Psi' = \unboxc{t} $}
    \prf{$\Gamma\vdash \Psi : \ctx$ \hfill by assumption}
    \prf{$\Gamma ; \Psi \vdash \id_{\unboxc{t}} : \unboxc{t}$\hfill by rule}
    \pcase{$\Psi' = \Psi_1, x{:}A$}
    \prf{$\Gamma;\Psi \vdash \sigma_1 : \Psi_1$}
    \prf{$\Gamma; \Psi \vdash x{:}A$ \hfill by rule}
    \prf{$\Gamma; \Psi \vdash x{:}[\sigma_1]A$ \hfill by rule}
    \prf{$\Gamma\vdash \Psi$\hfill by assumption}
    \prf{$\Gamma;\Psi\vdash \sigma, x : \Psi' $\hfill by rule}
  \item
    \prf{$\Gamma \vdash \Psi \equiv \Psi : \ctx$ and $\Gamma\vdash A\equiv B$ \hfill by inversion}
    \prf{$\Gamma\vdash \Psi : \ctx$ \hfill by Lemma}



  \item TODO
 %   By induction on the derivation.\\
  %  \pcase{\ianc{\Gamma \vdash \Psi : \ctx}{\Gamma \vdash \Psi \equiv \Psi : \ctx}{}}
  %  \prf{$\Gamma;\Psi \vdash \sigma : \Psi$\hfill by part 1.}
  %  \pcase{\ianc{\Gamma \vdash \Phi \equiv \Psi : \ctx}{\Gamma \vdash \Psi \equiv \Phi : \ctx}{}}
  %  \prf{$\Gamma; \Psi \vdash \sigma : \Phi$ \hfill by IH}
   % \prf{$\Gamma; \Phi \vdash \sigma' : \Psi$ \hfill by IH}
%    \pcase{\ibnc{\Gamma \vdash \Psi_1 \equiv \Psi_3 : \ctx}{\Gamma \vdash \Psi_3 \equiv \Psi_2 : \ctx}{\Gamma \vdash \Psi_1 \equiv \Psi_2 : \ctx}{}}
%    \prf{$\Gamma; \Psi_1 \vdash \sigma_{1,3} : \Psi_3$ \hfill by IH}
%    \prf{$\Gamma; \Psi_3 \vdash \sigma_{3,1} : \Psi_1$ \hfill by IH}
%    \prf{$\Gamma; \Psi_3 \vdash \sigma_{3,2} : \Psi_2$ \hfill by IH}
%    \prf{$\Gamma; \Psi_2 \vdash \sigma_{2,3}: \Psi_3$ \hfill by IH}
%    \prf{$\Gamma; \Psi_1 \vdash [\sigma_{1,3}]\sigma_{3,2} : \Psi_2$ \hfill by Lemma}
%    \prf{$\Gamma; \Psi_2 \vdash [\sigma_{2,3}]\sigma_{3,1} : \Psi_1$ \hfill by Lemma}
%    \pcase{\ibnc{\Gamma \vdash \Psi \equiv \Phi : \ctx}{\Gamma; \Psi \vdash A \equiv B : \lftype}{\Gamma \vdash \Psi, x{:}A \equiv \Phi,x {:}B : \ctx}{}}
%    \prf{$\Gamma; \Psi \vdash \sigma : \Phi$ \hfill by IH}
%    \prf{$\Gamma; \Phi \vdash \sigma' : \Psi$ \hfill by IH}
%
%    \prf{$\Gamma \vdash \Psi, x {:}A : \ctx$ \hfill TODO}
%    \prf{$\Gamma \vdash \Phi, x{:}B : \ctx$ \hfill TODO}
%    \prf{$\Gamma; \Psi, x{:}A \vdash \sigma : \Phi$ \hfill by IH}
%    \prf{$\Gamma; \Phi, x{:}B \vdash \sigma' : \Psi$ \hfill by IH}
%    \prf{$\Gamma; \Psi, x {:} A \vdash x : A$ \hfill by rule}
%    \prf{$\Gamma; \Phi, x {:} B \vdash x : B$ \hfill by rule}



%    \prf{ NEED TO PROVE THAT [\sigma]B  = A and inverse}
%    \prf{$\Gamma; \Psi, x {:}A \vdash \sigma, x : \Phi, x {:} B$ \hfill by IH}
%    \prf{$\Gamma; \Phi, x {:}B \vdash \sigma', x : \Psi, x {:}A$ \hfill by IH}}

  \end{enumerate}
\end{proof}



\begin{lemma}
  If $\Gamma, \Psi \vdash ?? \equiv ?? : ??$ then $\Gamma\vdash \Psi : \ctx$
\end{lemma}

\begin{proof}
  TODO
\end{proof}
\begin{theorem}
  \begin{enumerate}
    \item If $\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x C D : \lftype$
      then $\Gamma; \Psi \vdash A \equiv C : \lftype$
    \item If $\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x C D : \lftype$
      then $\Gamma; \Psi, x: A \vdash B \equiv D : \lftype$
  \end{enumerate}
\end{theorem}

\begin{proof}
  By induction on the derivation.\\
  \begin{enumerate}
  \item
    By induction on the derivation.\\
    \pcase{\ianc{\Gamma; \Psi \vdash \Pityp x A B : \lftype}{\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x C D : \lftype}{}}
    \prf{$\Gamma; \Psi \vdash A : \lftype$ \hfill by inversion}
    \prf{$\Gamma; \Psi \vdash A \equiv A : \lftype$ \hfill by rule}
    %
    \pcase{\ianc{\Gamma; \Psi \vdash \Pityp x C D \equiv \Pityp x A B: \lftype}{\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x C D : \lftype}{}}
    \prf{$\Gamma; \Psi \vdash B \equiv A : \lftype$ by IH}
    \prf{$\Gamma; \Psi \vdash A \equiv B : \lftype$ by rule}
    %
    \pcase{\ibnc{\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x E F : \lftype}{\Gamma; \Psi \vdash \Pityp x E F \equiv \Pityp x C D : \lftype}{\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x C D : \lftype}{}}
    \prf{$\Gamma; \Psi \vdash A \equiv E : \lftype$ \hfill by IH}
    \prf{$\Gamma; \Psi \vdash E \equiv C : \lftype$ \hfill by IH}
    \prf{$\Gamma; \Psi \vdash A \equiv C : \lftype$\hfill by rule}
    %
    \pcase{\ibnc{\Gamma; \Psi \vdash A \equiv C : \lftype}{\Gamma; \Psi, x : A \vdash B \equiv D : \lftype}{\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x C D : \lftype}{}}
  \item
    \pcase{\ianc{\Gamma; \Psi \vdash \Pityp x A B : \lftype}{\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x C D : \lftype}{}}
    \prf{$\Gamma; \Psi, x : A \vdash B : \lftype$ \hfill by inversion}
    \prf{$\Gamma; \Psi, x : A \vdash B \equiv B: \lftype$ \hfill by rule}
    %
    \pcase{\ianc{\Gamma; \Psi \vdash \Pityp x C D \equiv \Pityp x A B: \lftype}{\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x C D : \lftype}{}}
    \prf{$\Gamma; \Psi, x : C \vdash D \equiv B : \lftype$ \hfill by IH}
    \prf{$\Gamma; \Psi, x : C \vdash B \equiv D : \lftype$ \hfill by rule}
    \prf{$\Gamma \vdash \Psi : \ctx$ \hfill by Lemma \ref{}}
    \prf{$\Gamma; \Psi \vdash \sigma : \Psi$ \hfill by Lemma \ref{}}

    \prf{$\Gamma; \Psi\vdash A : \lftype$ \hfill by NEEDED}
    \prf{$\Gamma \vdash \Psi, x {:}A : \Psi$ \hfill by Lemma \ref{}}
    \prf{$\Gamma; \Psi, x{:}A \vdash \sigma : \Psi$ \hfill by Lemma \ref{}}
    \prf{$\Gamma \vdash  \Psi, x{:}A$ \hfill by Lemma \ref{}}
    \prf{$\Gamma, \Psi, x{:}A \vdash x : A$ \hfill by rule}
    \prf{$\Gamma, \Psi, x{:}A \vdash x : B$ \hfill by rule}
    \prf{$\Gamma \Psi, x {:} A \vdash \sigma : \Psi, x{:}B$ \hfill by rule}
    \prf{$\Gamma; \Psi, x : A \vdash B \equiv D : \lftype$ \hfill }
    %
    \pcase{\ibnc{\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x E F : \lftype}{\Gamma; \Psi \vdash \Pityp x E F \equiv \Pityp x C D : \lftype}{\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x C D : \lftype}{}}
    \prf{$\Gamma; \Psi, x{:}A\vdash B \equiv F : \lftype$ \hfill by IH}
    \prf{$\Gamma; \Psi, x{:}E\vdash F \equiv D : \lftype$ \hfill by IH}
    \prf{$\Gamma; \Psi \vdash A \equiv E$ \hfill by 1.}
    \prf{$\Gamma \vdash \Psi : \ctx$ \hfill by Lemma \ref{}}
    \prf{$\Gamma; \Psi \vdash \sigma : \Psi$ \hfill by Lemma \ref{}}
    \prf{$\Gamma \vdash \Psi, x {:}A : \ctx$ \hfill by Lemma \ref{}}
    \prf{$\Gamma ; \Psi \vdash A : \lftype$ \hfill by inversion}
    \prf{$\Gamma \vdash \Psi, x {:}A : \Psi$ \hfill by Lemma \ref{}}
    \prf{$\Gamma; \Psi, x{:}A \vdash \sigma : \Psi$ \hfill by Lemma \ref{}}
    \prf{$\Gamma, \Psi, x{:}A \vdash x : A$ \hfill by rule}
    \prf{$\Gamma, \Psi, x{:}A \vdash x : E$ \hfill by rule}
    \prf{$\Gamma \Psi, x {:} A \vdash \sigma : \Psi, x{:}E$ \hfill by rule}
    \prf{$\Gamma; \Psi, x{:}A\vdash F \equiv D : \lftype$ \hfill by IH}
    \prf{$\Gamma; \Psi, x{:}A\vdash B \equiv D : \lftype$ \hfill by IH}
    %
    \pcase{\ibnc{\Gamma; \Psi \vdash A \equiv C : \lftype}{\Gamma; \Psi, x : A \vdash B \equiv D : \lftype}{\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x C D : \lftype}{}}
  \end{enumerate}
\end{proof}







\begin{lemma}
  If $\Gamma \vdash (\hatctx{\Psi} \vdash A) \equiv (\hatctx{\Psi} \vdash B)$ then $\Gamma ; \Psi \vdash A \equiv B :\lftype $
\end{lemma}


\begin{proof}
  \pcase{\ianc{\Gamma \vdash (\Psi \vdash A)}{\Gamma \vdash (\hatctx{\Psi} \vdash A) \equiv (\hatctx{\Psi} \vdash A)}{}}
  \prf{$\Gamma \vdash (\hatctx{\Psi} \vdash A)$ \hfill by assumption}
  \prf{$\Gamma ; \Psi \vdash A : \lftype$ \hfill by inversion}
  \prf{$\Gamma ; \Psi \vdash A \equiv A: \lftype$ \hfill by rule}
  \pcase{\ibnc{\Gamma \vdash (\hatctx{\Psi} \vdash A) \equiv (\hatctx{\Psi} \vdash C)}{\Gamma \vdash (\hatctx{\Psi} \vdash C) \equiv (\hatctx{\Psi} \vdash B)}{\Gamma \vdash (\hatctx{\Psi} \vdash A) \equiv (\hatctx{\Psi} \vdash B)}{}}
  \prf{$\Gamma ; \Psi \vdash A \equiv C$ \hfill by IH}
  \prf{$\Gamma ; \Psi \vdash C \equiv B$ \hfill by IH}
  \prf{$\Gamma ; \Psi \vdash A \equiv B$ \hfill by rule}
  \pcase{\ianc{\Gamma \vdash (\hatctx{\Psi} \vdash B) \equiv (\hatctx{\Psi} \vdash A)}{\Gamma \vdash (\hatctx{\Psi} \vdash A) \equiv (\hatctx{\Psi} \vdash B)}{}}
  \prf{$\Gamma ; \Psi \vdash B \equiv A$ \hfill by IH}
  \prf{$\Gamma ; \Psi \vdash A \equiv B$ \hfill by rule}
  \pcase{\ianc{\Gamma ; \Psi \vdash A \equiv B}{\Gamma \vdash (\hatctx{\Psi} \vdash A) \equiv (\hatctx{\Psi} \vdash B)}{}}
  \prf{$\Gamma ; \Psi \vdash B \equiv A$ \hfill by IH}
  \prf{$\Gamma ; \Psi \vdash A \equiv B$ \hfill by rule}
\end{proof}











\begin{lemma}
  \begin{enumerate}
    \item   If $\Gamma \vdash \Psi_1 \equiv \Psi_2 : \ctx$ and $\Psi_1 \lfwhnf \Phi_2$ then $\Psi_1 \lfwhnf \Phi_2$
  \item
    If $\Gamma \vdash \Psi_1 \equiv \Psi_2 : \ctx$ and $\Psi_1 \lfwhnf \Phi_2$ then $\Psi_1 \lfwhnf \Phi_2$
  \end{enumerate}
\end{lemma}
\begin{proof}
  \begin{enumerate}
  \item
    \pcase{\ianc{\norm \Psi_1'}{\norm (\Psi_1' , x:A)}{}}
    \prf{$\Psi_2 = \Psi_2', x :B$\hfill by construction}
    \prf{$\norm \Psi_2'$ \hfill by IH}
    \prf{$\norm \Psi_2', x: B$ \hfill by rule}
    \pcase{\ianc{}{\norm \cdot}{}}
    \prf{$\Psi_2 = \cdot$}
    \pcase{\ianc{\neut t}{\norm {\unboxc{t}}}{}}
    \prf{$\Psi_1 = \Psi_2$ \hfill by construction}%%SEE IF WE CHANGE IT
  \item
    \pcase{\ianc{\Psi_1' \lfwhnf \Phi_1}{\Psi_1', x{:}A \lfwhnf \Phi_1', x{:}A}{}}
    \prf{$\Gamma\vdash \Psi_1' \equiv \Psi_2'$ \hfill by inversion and $\Psi_2 = \Psi_2', x {:}B$}
    \prf{$\Psi_2' \lfwhnf \Phi_2'$ \hfill by IH}
    \prf{$\Psi_2',x {:}B \lfwhnf \Phi_2', x{:}B$ \hfill by rule}
    \pcase{\ibnc{t \whnf \cbox{\Phi}}{\Phi \lfwhnf \Psi}{\unboxc{t} \lfwhnf \Psi}{}}
    \prf{$\Psi_1= \Psi_2$}
    \pcase{\ianc{\norm \Psi_1}{\Psi_1 \lfwhnf \Psi_1}{}}
    \prf{$\norm \Psi_2$ \hfill by part 1.}
    \prf{$\Psi_2 \lfwhnf \Psi_2$ \hfill by rule}
  \end{enumerate}

\end{proof}











%I think we should change the equivalence for (Psi |-A) and (Psi|-M)
%

\begin{lemma}
  \begin{itemize}
  \item If $\Gamma \Vdash C : T$ and $\Gamma \vdash T \equiv T'$  then $\Gamma \Vdash C :T'$
  \item If $\Gamma; \Psi \Vdash M : A$ and $\Gamma; \Psi \vdash A \equiv B :\lftype$ then $\Gamma ; \Psi \Vdash M : B$
  \end{itemize}
  \end{lemma}




\begin{proof}
  By induction on the first derivation.\\
  \pcase{$\Gamma; \Psi \vdash M : \tm$}
  \prf{$\Gamma; \Psi \vdash \tm \equiv \tm : \lftype$ is the only possibility by def. of equivalence}
  %
  \pcase{\ianc{\forall N.~\Gamma ; \Psi \Vdash N : A \Longrightarrow \Gamma ; \Psi \vdash M~N : [N/x]B}{\Gamma ; \Psi \Vdash M : \Pi x{:}A. B}{}}
  \prf{$\Gamma; \Psi \vdash \Pityp x A B \equiv \Pityp x C D : \lftype$ \hfill by definition of equivalence}
  \prf{Assume that $\Gamma; \Psi \Vdash N : C $}
  \prf{$\Gamma; \Psi \vdash A \equiv C : \lftype$ \hfill by Lemma \ref{}}
  \prf{$\Gamma ; \Psi \vdash [N/x]B \equiv [N/x]D$\hfill by Lemma \ref{}}
  \prf{$\Gamma \Vdash N : A$ \hfill by IH}
  \prf{$\Gamma ; \Psi \vdash M~N : [N/x]B$ \hfill by construction}
  \prf{$\Gamma ; \Psi \vdash M~N : [N/x]D$ \hfill IH}
  \prf{$\Gamma ;  \Psi \Vdash M : \Pi x {:}A.B$ \hfill by definition}
  %
  \pcase{$\Gamma \Vdash \Psi : \tmctx$}
  \prf{$\Gamma \vdash \tmctx \equiv \tmctx$ is the only possibility by def. of equivalence}
  %
  \pcase{\ianc{\Gamma ; \Psi \Vdash M : A}{\Gamma \Vdash (\hatctx{\Psi} \vdash M) : (\Psi \vdash A)}{}}
  \prf{$\Gamma \vdash (\Psi \vdash A) \equiv (\Psi \vdash B)$ \hfill by def. of equivalence}
  \prf{$\Gamma ; \Psi \vdash A \equiv B $ \hfill by Lemma \ref{}}
  \prf{$\Gamma; \Psi \Vdash M : B$ \hfill by IH}
  \prf{$\Gamma\Vdash (\hatctx{\Psi} \vdash M) : (\Psi \vdash B)$ \hfill by rule}

\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:






















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{lemma}[Semantic Type Conversion]\quad
  \begin{enumerate}
  \item If $\Gamma \Vdash T \equiv T'$ and $\Gamma \Vdash C : T$ then
    $\Gamma \Vdash C : T'$.
  \item If $\Gamma \Vdash \tau \equiv \tau'$ and $\Gamma \Vdash t : \tau$ then $\Gamma \Vdash t : \tau'$.
  \end{enumerate}

\end{lemma}

\begin{proof}
  By induction on $\Gamma \Vdash \tau$.
\\[1em]
\pcase{$\D = \ibnc{\tau \whnf \cbox{T}}
         {\forall \Gamma' \leq_\rho \Gamma.~\Gamma' \Vdash \{\rho\}T }
         {\Gamma \Vdash \tau}{}$}
\prf{$\Gamma \Vdash t : \cbox {T_1}$ \hfill by assumption}
\pcase{$\Gamma \vdash t \whnf \cbox C : \cbox{T_1}$ and $\Gamma   \Vdash C : T_1$ \hfill by semantic def.}
\prf{$\Gamma \Vdash \cbox{T_1}\equiv \tau'$ \hfill by assumption}
\prf{$\Gamma \vdash \tau' \whnf \cbox{T_2}$ and $\Gamma \vdash T_1  \equiv T_2$ \hfill by semantic def.}
\prf{$\Gamma\vdash t : \cbox{T_1}$\hfill by definition of $\Gamma \vdash t \whnf \cbox C : \cbox{T_1}$}
  \prf{$\Gamma\vdash t : \cbox{T_2}$\hfill by rule}
  \prf{$\Gamma\vdash \cbox C : \cbox{T_1}$\hfill by definition of $\Gamma \vdash t \whnf \cbox C : \cbox{T_1}$}
  \prf{$\Gamma\vdash \cbox C : \cbox{T_2}$\hfill by rule}
  \prf{$\Gamma \vdash t \equiv \cbox C : \cbox{T_1}$ \hfill by definition of $\Gamma \vdash t \whnf \cbox C : \cbox{T_1}$}
  \prf{$\Gamma \vdash t \equiv \cbox C : \cbox{T_2}$ \hfill by rule}
  \prf{$t \whnf \cbox C$ \hfill by definition of $\Gamma \vdash t \whnf \cbox C : \cbox{T_1}$}
  \prf{$\Gamma \vdash t \whnf \cbox C : \cbox{T_2}$ \hfill by definition}
  \prf{$\Gamma\Vdash C : T_2$ \hfill by IH}
  \prf{$\Gamma \Vdash t : \cbox{T_2}$ \hfill by definition}
\\[0.5em]
  %subcase
  \pcase{$\Gamma \vdash t \whnf n : \cbox{T_1}$ and $\neut n$}
  \prf{$\Gamma\Vdash \cbox{T_1}\equiv \tau$ \hfill by  assumption}
\prf{$\Gamma \vdash \tau' \whnf \cbox{T_2}$ and $\Gamma \vdash T_1  \equiv T_2$ \hfill by semantic def.}
  \prf{$\Gamma\vdash t : \cbox{T_1}$\hfill by definition of $\Gamma \vdash t \whnf n : \cbox{T_1}$}
  \prf{$\Gamma\vdash t : \cbox{T_2}$\hfill by rule}
  \prf{$\Gamma\vdash n: \cbox{T_1}$\hfill by definition of $\Gamma \vdash t \whnf n : \cbox{T_1}$}
  \prf{$\Gamma\vdash n : \cbox{T_2}$\hfill by rule}
  \prf{$\Gamma \vdash t \equiv n : \cbox{T_1}$ \hfill by definition of $\Gamma \vdash t \whnf n : \cbox{T_1}$}
  \prf{$\Gamma \vdash t \equiv n : \cbox{T_2}$ \hfill by rule}
  \prf{$t \whnf n$ \hfill by definition of $\Gamma \vdash t \whnf n : \cbox{T_1}$}
  \prf{$\Gamma \vdash t \whnf n : \cbox T_1$ \hfill by definition}
  \prf{$\neut n$ \hfill by definition}
  \prf{$\Gamma \Vdash t : \cbox{T_2}$ \hfill by definition}
  %
\\[0.5em]
  \pcase{$\D = \ianc{ \tau \whnf (y:\tau_1) \arrow \tau_2 \quad
(\forall \Gamma' \leq_\rho \Gamma. \Gamma' \Vdash \{\rho\}\tau_1 :{ \flagred{u_1}}) \quad
  \forall \Gamma' \leq_\rho \Gamma. \Gamma \Vdash t : \{\rho\}\tau_1  :{ \flagred{u_1}}
   \Longrightarrow \Gamma' \Vdash \{\rho, t/x\} \tau_2 : {\flagred{u_2}} }
         {\Gamma \Vdash \tau \flagred{: u_3}}{}$ }
  \prf{where $~ \flagred{(u_1, u_2, u_3) \in \mathcal{R}}$}
  \prf{$\Gamma \Vdash t : (y:\tau_1) \arrow \tau_2$ \hfill by assumption}
  \prf{$\Gamma\Vdash (y:\tau_1) \arrow \tau_2 = (y:\tau_1') \arrow \tau_2'$ \hfill by assumption}
  \prf{$\forall \Gamma' \leq_\rho \Gamma.~\Gamma' \Vdash \{\rho\}\tau_1 = \{\rho\}\tau'_1$ \hfill by semantic def.}
  \prf{$\forall \Gamma' \leq_\rho \Gamma.~\Gamma' \Vdash s = s' : \{\rho\}\tau_1 \Longrightarrow \Gamma' \Vdash \{\rho, s/y\}\tau_2 = \{\rho, s'/y\}\tau'_2$ \hfill by semantic def.}
  \prf{$\Gamma\vdash (y:\tau_1) \arrow \tau_2 \equiv (y:\tau_1') \arrow \tau_2'$ \hfill by Lemma \ref{lm : semsyntypeq}}
  \prf{$\Gamma \vdash t \whnf w : (y:\tau_1) \arrow \tau_2$ \hfill by semantic def.}
  \prf{$\Gamma \vdash t :  (y:\tau_1) \arrow \tau_2 $ \hfill by Def. \ref{def:typedwhnf}}
  \prf{$\Gamma \vdash t :  (y:\tau_1') \arrow \tau_2' $ \hfill by rule}
  \prf{$\Gamma \vdash w :  (y:\tau_1) \arrow \tau_2 $ \hfill by Def. \ref{def:typedwhnf}}
  \prf{$\Gamma \vdash w :  (y:\tau_1') \arrow \tau_2' $ \hfill by rule}
  \prf{$\Gamma \vdash t \equiv w :  (y:\tau_1) \arrow \tau_2 $ \hfill by Def. \ref{def:typedwhnf}}
  \prf{$\Gamma \vdash t \equiv w :  (y:\tau_1') \arrow \tau_2' $ \hfill by rule}
  \prf{$t \whnf w$ \hfill by def}
  \prf{$\Gamma \vdash t \whnf w : (y:\tau_1') \arrow \tau_2'$ \hfill by Def. \ref{def:typedwhnf}}
  \prf{Assume that $\Gamma' \leq_\rho \Gamma$ and $\Gamma' \Vdash t' :  \{\rho\}\tau_1'$}
  \prf{\mbox{$\quad$}$\Gamma'\Vdash\{\rho\}\tau_1 = \{\rho\}\tau'_1$ \hfill by previous lines}%verify it is possible
  \prf{\mbox{$\quad$}$\Gamma'\Vdash\{\rho\}\tau'_1 = \{\rho\}\tau_1$ \hfill by symmetry of semantic definitions (Lemma \ref{lem:semsym})}%verify it is possible
  \prf{\mbox{$\quad$}$\Gamma' \Vdash t' : \{\rho\}\tau_1$ \hfill by IH}
  \prf{\mbox{$\quad$}$\Gamma' \Vdash t' = t' :  \{\rho\}\tau_1$ \hfill by reflexivity of semantic definitions}
  \prf{\mbox{$\quad$}$\Gamma' \Vdash \{\rho,t'/y\}\tau_2 = \{\rho, t'/y\}\tau'_2$ \hfill by previous lines}
  \prf{\mbox{$\quad$}$\forall \Gamma' \leq_\rho \Gamma.~\Gamma' \Vdash t' : \{\rho\}\tau_1 \Longrightarrow \Gamma' \Vdash (\{\rho\}w)~t' : \{\rho, t'/y\}\tau_2$ \hfill by semantic def.}
\prf{\mbox{$\quad$}$\Gamma' \Vdash (\{\rho\}w)~t' : \{\rho, t'/y\}\tau_2$ \hfill by previous lines}
\prf{\mbox{$\quad$}$\Gamma' \Vdash (\{\rho\}w)~t' : \{\rho, t'/y\}\tau'_2$ \hfill by IH}
  \prf{$\Gamma \Vdash t : (y:\tau_1') \arrow \tau_2'$ \hfill by construction}
 \end{proof}







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

